Low-Power Status Updates via Sleep-Wake Scheduling

We consider the problem of optimizing the freshness of status updates that are sent from a large number of low-power sources to a common access point. The source nodes utilize carrier sensing to reduce collisions and adopt an asynchronized sleep-wake scheduling strategy to achieve a target network lifetime (e.g., 10 years). We use age of information (AoI) to measure the freshness of status updates, and design sleep-wake parameters for minimizing the weighted-sum peak AoI of the sources, subject to per-source battery lifetime constraints. When the sensing time (i.e., the time duration of carrier sensing) is zero, this sleep-wake design problem can be solved by resorting to a two-layer nested convex optimization procedure; however, for positive sensing times, the problem is non-convex. We devise a low-complexity solution to solve this problem and prove that, for practical sensing times that are short, the solution is within a small gap from the optimum AoI performance. When the mean transmission time of status-update packets is unknown, we devise a reinforcement learning algorithm that adaptively performs the following two tasks in an ``efficient way'': a) it learns the unknown parameter, b) it also generates efficient controls that make channel access decisions. We analyze its performance by quantifying its ``regret'', i.e., the sub-optimality gap between its average performance and the average performance of a controller that knows the mean transmission time. Our numerical and NS-3 simulation results show that our solution can indeed elongate the batteries lifetime of information sources, while providing a competitive AoI performance.

==> learning_Jan_14.tex <==
\begin{flushleft}
\textbf{Regret when} $\bm{|\te\ust - \hat{\te}(\tau_k)|< \delta}$: 
\end{flushleft}
Choose a sufficiently large $k_0\in \bN$, and define the following event
\begin{align*}
\cG_3 :=  \cap_{k \ge k_0 } \cG_3(\tau_k).
\end{align*}
It follows from Lemma~\ref{lemma:g2}, and union bound, that $\cG_3$ has a probability greater than $1- \sum_{k>k_0} \exp(-\delta_1 \tau_k)$. On $\cG_3$, the number of samples $N(\tau_k)$ at the beginning of each episode $k>k_0$ is greater than $\left(p_{\min} -  \sqrt{\delta_1}\right)\tau_k$. Thus on $\cG_3$, for episodes $k>k_0$ the radius of $\cC(\tau_k)$ is less than $\sqrt{\frac{\log H^{\gamma}}{(p_{\min}- \sqrt{\delta_1})\tau_k }}$. Let $k_1$ be the smallest integer greater than $k_0$ that satisfies
\begin{align}\label{ineq:radius}
\frac{\log H^{\gamma}}{( p_{\min} - \sqrt{\delta_1})\tau_{k_{1} }}\le \delta^{2},
\end{align} 
where the constant $\delta>0$ is as in Lemma~\ref{lemma:convergence}. Thus, on $\cG_3$, for episodes $k\ge \max \left\{ k_0, k_1 \right\}$, the radius of confidence intervals is less than $\delta$. Note that on $\cap_{k}\cG_1(\tau_k)$ the confidence intervals~\eqref{def:ucb_ci} at the beginning of each episode are true. Hence, on $\cap_{k}\cG_1(\tau_k) \cap \cG_3$ we have $| \hat{\te}(\tau_k) - \te\ust |<\delta$ for epsiodes $k\ge \max \left\{ k_0, k_1 \right\}$. Thus, on $\cap_{k}\cG_1(\tau_k) \cap \cG_3$ cumulative regret is bounded by $K_2 \max\left\{\tau_{k_0},\tau_{k_1}\right\}$. 

The probability of failure of $\cC(\tau_k)$ is less than $\frac{1}{\tau^{\gamma -1}_k}$ (Lemma~\ref{lemma:g1}); moreover since the episode duration of $\cE_k$, $(\tau_{k+1} - \tau_k )$ is less than $\tau_k$, we have that the expected value of the regret in the event of failure of $\cC(\tau_k)$ is less than $K_2 \frac{1}{\tau^{\gamma - 2}_k}$. \textcolor{red}{Since $\gamma>3~or~4?$}, the cumulative expected regret $K_2 \sum_k \frac{1}{\tau^{\gamma - 2}_k}$ is finite. In summary, the first summation in~\eqref{def:reg_dec} is upper-bounded by $K_2\frac{\log H^{\gamma}}{( p_{\min} - \sqrt{\delta_1})  \delta^{2}}$. This discussion is summarized as the following result.
\begin{lemma}
Under Algorithm~\ref{algo:ucb} the following is true, 
\begin{align}
\sum_{k=1}^{K} \left(\tau_{k+1} - \tau_k  \right) \bP( | \hat{\te}(\tau_k) - \te\ust |>\delta ) \le K_2\frac{\log H^{\gamma}}{( p_{\min} - \sqrt{\delta_1})  \delta^{2}}.
\end{align}


\end{lemma}


==> sections/Discussion.tex <==
\section{Discussion}\label{Disc}
In this section, we discuss our results and compare it with prior works. 
\subsection{Preemption vs. Non-Preemption}
In the conclusion of \cite[Appendix]{CostaCodreanuEphremides_TIT}, the authors claimed that "In  the  LCFS  system  with  preemption  we  expect  that,  for  very large  arrival  rates,  the  age  would  increase  without  bound,  as  no  packet  finishes  service''. This claim is correct when the packet service times are NBU. As we will see in Fig. \ref{avg_peak_age3}, the age of the preemptive LCFS policy grows to infinity at high traffic intensity for gamma distributed service times. However, preemption does not increase the age for exponential service times, because the remaining service times of a preempted packet has the same distribution with the service time of a new packet. In Theorem \ref{thm1}, we have proven that the preemptive LCFS policy is age-optimal for exponential service times and general system parameters. In Theorem 3(a) of \cite{RYatesTIT16}, Yates and Kaul showed that the average age of the preemptive LCFS policy is a decreasing function of the traffic intensity $\rho$ in M/M/1 queues as $\rho$ grows to infinite. 

%On one hand, this contradicts our results in Theorem \ref{thm1}, in which we showed that the LCFS system with preemption can, indeed, achieve age-optimality for all arrival rates among all causal policies when the service times are exponentially distributed and the update packets arrive in the order of their generation times. Moreover, the study in \cite{RYatesTIT16} showed that the preemptive LCFS policy achieves bounded average age for all arrival rates when the service times are exponentially distributed. However, for non-exponential service time, the age of the preemptive LCFS policy could blow up at high traffic intensity (as we will see in Fig. \ref{avg_peak_age3}). This is because the packet service times are no longer memoryless. Thus, high traffic intensity leads to increased preemption rate which, in turn, leads to no packet completes service. Hence, the inter-departure times increase causing the rise in the age. From this, we can deduce that the age performance of the prmp-LGFS-R policy depends essentially on the service time distribution.

In addition, the study in \cite{Gamma_dist} characterized the age for LCFS systems with and without preemption for  gamma distributed service times. In \cite[Numerical Results]{Gamma_dist}, the authors showed that the non-preemptive LCFS policy can achieve better average age performance than the preemptive LCFS policy. In this paper, we further show that the non-prmp-LGFS-R policy is within a small constant gap from the optimum expected average age for all NBU service time distributions, which include gamma distribution as one example.

%In addition, the study in \cite{Gamma_dist} characterized the age for LCFS systems with and without preemption when the service time is gamma distributed (gamma distribution belongs to the class of NBU distributions). In \cite[Numerical Results]{Gamma_dist}, the authors showed that the non-preemptive policy can achieve better average age than the preemptive one. In this paper, we showed that the non-prmp-LGFS-R policy can come close to age-optimal when the service time is NBU distributed. More specifically, the non-prmp-LGFS-R is within a small age gap from the optimum expected average age for NBU service times.

\subsection{Replication vs. Non-Replication}
The replication technique has gained significant attention in recent years to reduce the delay in queueing systems \cite{Chen_queue_coding,yin_data_retrieve,sun2016delay}. However, under some system settings, replications may worsen the delay performance. In particular, it was shown in \cite{sun2016delay} that replication policies are far from the optimum delay for NBU service time distributions. A simple explanation of this result is as follows: Let $X_1, X_2, \ldots, X_m$ be i.i.d. NBU random variables with mean $\mathbb{E}[X_l]=\mathbb{E}[X]<\infty$. From the properties of the NBU distributions, we can obtain \cite{joshi2017efficient}
\begin{equation}\label{NBUproperty_delay}
\mathbb{E}[\min_{l=1,\ldots,m}X_l]\geq \frac{\mathbb{E}[X]}{m}.
\end{equation}
Now, if $X_l$ represents the packet service time of server $l$, then the left-hand side of \eqref{NBUproperty_delay} represents the mean service time (the mean time spent by each server per packet) when each packet is replicated to all servers; and the right-hand side of \eqref{NBUproperty_delay} represents the mean service time when there is no replication. This gives insight why packet replication can worsen the delay performance when the service time is NBU. Somewhat to our surprise, we found in this paper that the non-prmp-LGFS-R policy is near-optimal in minimizing the age, even for NBU service time distributions. The intuition behind this result is that the age is affected by the freshness of the delivered packets irrelevant to the total number of delivered packets. In other words, to reduce the age, we need to deliver the freshest packet as soon as possible. Also, it is obvious that 
\begin{equation}
\mathbb{E}[\min_{l=1,\ldots,m}X_l]\leq\mathbb{E}[X].
\end{equation}
Thus, packet replication can help in this direction by exploiting the diversity provided by multiple servers. 
\subsection{New-Worse-than-Used service time distributions}
Another important class of distributions that are more general than exponential is New-Worse-than-Used (NWU) distributions. The definition of the NWU distributions is as follows: 
\begin{definition}  \textbf{New-Worse-than-Used distributions:} Consider a non-negative random variable $Z$ with CCDF $\bar{F}(z)=\mathbb{P}[Z>z]$. Then, $Z$ is \textbf{New-Worse-than-Used (NWU)} if for all $t,\tau\geq0$
\begin{equation}\label{NWU_Inequality}
\bar{F}(\tau +t)\geq \bar{F}(\tau)\bar{F}(t).
\end{equation} 
\end{definition}
Examples of NWU distributions include hyperexponential distribution, Weibull distribution with $c <1$, etc. A  random variable is both NBU and NWU if, and only if, it is exponential. We investigated whether age-optimality can be achieved when the service times are NWU. We figured out that no policy can achieve optimality when the service times are NWU. To clarify this claim, let us consider the following example.

 \begin{figure*}[!tbp]
 \centering
 \subfigure[Case 1: Preemption is allowed.]{
  \includegraphics[scale=0.3]{figure/NWU.eps}
   \label{1a}
   }
 \subfigure[Case 2: Preemption is not allowed.]{
  \includegraphics[scale=0.3]{figure/NWU2.eps}
   \label{2b}
   }
   \caption{Illustration of policies $\pi$ and $\pi'$ in the Example }
   \label{fig:samp_path_NBU}
\end{figure*}
\textbf{Example:}
\emph{Consider a single server queue with $U(0)=0$ for all policies. We first consider the case where preemption is allowed. Suppose that the policies $\pi$ and $\pi'$ start to process packet 1 at time 0, as shown in  Fig. \ref{1a}. Suppose that at time $\delta$, packet 2 with $s_2<s_1$ arrives at the system. Since $s_1>s_2$, an intuitive action is to keep processing the fresh packet (packet 1) and ignore the old packet (packet 2). We will show that this decision may not achieve lower age. Suppose that policy $\pi'$ preempts the processing of packet 1 and starts to serve packet 2 at time $\delta$ and completes the service of packet 2 at time $\gamma$, as shown in  Fig. \ref{1a}. Let $R_1$ represent the remaining service time to complete packet 1 at time $\delta$ under policy $\pi$. Suppose that the server has spent $\chi$ ($\chi\geq 0$) seconds on processing packet 1 by time $\delta$ in policy $\pi$. Define $X_1=\chi+R_1$ as the service time of packet 1 under policy $\pi$ and $X_2=\gamma-\delta$ as the service time of packet 2 under policy $\pi'$. Then, the CCDF of $R_1$ is given by
\begin{equation}\label{ex_NWU_1}
\mathbb{P}[R_1>t]=\mathbb{P}[(X_1-\chi)>t\vert X_1>\chi].
\end{equation}
Because the packet service times are NWU, we can obtain that for all $t, \chi\geq 0$
\begin{equation}\label{ex_NWU_2}
\mathbb{P}[(X_1-\chi)>t\vert X_1>\chi]=\mathbb{P}[(X_2-\chi_1)>t\vert X_2>\chi_1]\geq\mathbb{P}[X_2>t].
\end{equation}
Combining \eqref{ex_NWU_1} and \eqref{ex_NWU_2}, we get
\begin{equation}\label{ex_NWU_3}
R_1\geq_{\text{st}}X_2.
\end{equation}
This means that the completion time of packet 2 under policy $\pi'$ is stochastically smaller than the completion time of packet 1 under policy $\pi$, as shown in  Fig. \ref{1a}. Thus, policy $\pi'$ can obtain lower age at time $\gamma$ than policy $\pi$, i.e., we have
\begin{equation}
\Delta_\pi(\gamma)=\gamma\geq\gamma-s_2=\Delta_{\pi'}(\gamma).
\end{equation}}

\emph{Now, we proceed to the case where preemption is not allowed. We will show that a non-work-conserving policy can obtain lower age than the work-conserving one. Suppose that policy $\pi$ starts processing packet 1 at time 0; and policy $\pi'$ does idle the server until time $\delta$, then assigns packet 2 to the server, as shown in Fig. \ref{2b}. We assume here that $0=a_1<a_2\leq\delta$ and $s_2>s_1$. By the same argument as in the first case, we can show that the completion time of packet 2 under policy $\pi'$ is stochastically smaller than the completion time of packet 1 under policy $\pi$, as shown in Fig. \ref{2b}. This means that the non-work-conserving policy $\pi'$ can obtain a lower age than policy $\pi$.}

This example shows that age-optimality is extremely hard to be achieved within the policy space that includes all causal policies when the service times are NWU distributed. However, we showed in \cite{multihop_optimal} that optimality can be achieved for general service time in single server queues among all non-preemptive work-conserving policies.

==> sections/Numerical_results__rahul_singh_s_conflicted_copy_2019-08-02_.tex <==
\section{Numerical Results}\label{Simulations}
Throughout, we use ``Age-optimal scheduler'' to denote the sleep-wake scheduler with the sleep period paramters $r_l^{\star}$'s as in \eqref{r_f_b_gr_1}, \textcolor{red}{that was shown to be asymptotically optimal in Theorem ?? }. By ``Throughput-optimal scheduler'', we  refer to the sleep-wake algorithm of~\cite{chen2013life} that is known to achieve the optimal trade-off between the throughput and energy consumption. Also, we use ``Fixed-rate scheduler'' to denote the \textcolor{red}{sleep-wake scheduler ??} algorithm in which the sleep period parameters $r_l$'s are equal for all the sources, i.e., $r_l=k$ for all $l$, \textcolor{red}{ where the parameter $k$ has been chosen so as to satisfy the energy constraints of Problem \textbf{1} }. \textcolor{red}{We also compare the performance of the above mentioned algorithms against the lower bounds~\eqref{lower_bound_sum_bi_ge_1}, \eqref{lower_bound_sum_bi_le_1}, and hence use the term ``lower bound'' in order to denote these lower bounds.}

\textcolor{red}{Throughout, we let the mean transmission time $\mathbb{E}[T]=5$ ms.} The weights $w_l$'s attached to different sources \textcolor{red}{refer to equation in problem } are generated by sampling from a uniform distribution in the interval $[0, 10]$. Similarly, the target energy efficiencies $b_l$'s \textcolor{red}{ of the sources\slash batteries?} are generated by sampling from the uniform distribution within the range [0, 1]. 

%The energy consumption rate for each source while it is transmitting is equal to 24.75 mW. The initial battery levels and recharging rates are set to 
%$B_l\equiv 1200$ mAh, $R_l\equiv .22$ for all sources. The target lifetimes are chosen such that the target energy efficiencies $b_l$'s are randomly generated uniformly  within the range [0, 1]. \textcolor{red}{shouldnt it be other way around? }

\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{figure/comparison_life_add_no_users_10_vs_ration_2.eps}
\centering
%\captionsetup{justification=justified, font={small,onehalfspacing}}
\captionsetup{justification=justified}
\caption{Total weighted average peak age $\bar{\Delta}^{\text{peak}}(\mathbf{r})$ versus the ratio $\frac{t_s}{\mathbb{E}[T]}$ for an update system with $M=10$ sources.}
%\vspace{-.1in}
\label{peak_age_comp}
\end{figure}
\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{figure/comparison_life_add_vs_no_users.eps}
\centering
%\captionsetup{justification=justified, font={small,onehalfspacing}}
\captionsetup{justification=justified}
\caption{Total weighted average peak age $\bar{\Delta}^{\text{peak}}(\mathbf{r})$ versus the number of sources $M$.}
%\vspace{-.1in}
\label{peak_age_comp_num}
\end{figure}
We set the number of sources at $M=10$. 
Fig.~\ref{peak_age_comp} plots the total weighted average peak age $\bar{\Delta}^{\text{peak}}$ ~\eqref{t_avg_peak_age} as a function of the ratio $\frac{t_s}{\mathbb{E}[T]}$. The age-optimal scheduler is seen to outperform the throughput-optimal and fixed-rate schedulers. This is not surprising since the throughput-optimal had been designed in order to maximize the throughput, and not minimize the age.
Moreover, we also observe that the \textcolor{red}{performance} of the age-optimal scheduler converges to the lower bound as $t_s/\mathbb{E}[T]\to 0$. \textcolor{red}{This is in accordance with our result on the near-optimality of } \textcolor{red}{what ?}. Finally, we observe that the total weighted average peak age of all schedulers increases as the sensing time increases. This is \textcolor{red}{expected since an increase in the sensing time leads to an increase in the probability of packet collisions, which in turn increases the average age.}



We then scale the number of sources $M$, and plot $\bar{\Delta}^{\text{peak}}$ as a function of $M$ in Fig.~\ref{peak_age_comp_num}. The sensing time $t_s$ is fixed at $t_s=40~\mu$s. The age-optimal scheduler is shown to outperform the other schedulers uniformly for all values of $M$. As expected, the total weighted average peak age of each scheduler increases with $M$, \textcolor{red}{ since...why??}. The gap between \textcolor{red}{the performance of age-optimal scheduler and the lower bound increases with $M$}. \textcolor{red}{This is the case because, as shown in equation ??, the sub-optimality gap is a linear increasing function of the parameters $C_1$,$C_2$~\eqref{eq23thm3_1} and \eqref{eq29thm3_3}, and moreover $C_1,C_2$ are increasing functions of $M$.}

%As we can observe, our proposed sleep-wake algorithm outperforms the other two algorithms in both the cases. This is not surprising since the ``Life-add'' algorithm \textcolor{red}{of paper name..} was designed to maximize the throughput, and optimizing the throughput does not translate to optimizing the AoI. Moreover, in Figure \ref{peak_age_comp}, we observe that the total weighted average peak age for all algorithms increases as the sensing time increases. This is reasonable, as increasing the sensing time leads to an increase in the probability of packet collisions, and hence the age performances of these \textcolor{red}{is it all these algos?} algorithms deteriorate.

%while using the sleep-wake algorithm, we will set the rate parameters $r_l$ as in \eqref{r_f_b_gr_1}.
%We compare the performance of our proposed sleep-wake algorithm with the round robin \cite{li2013throughput,hsu2017scheduling,kadota2016minimizing,kadota2016minimizing_journal,jiang2018timely}. Under the round robin algorithm sources take turns in order to transmit their update packet. Thus, once a source obtains channel access, it transmits until its battery dies out. The execution of an algorithm is completed when all the sources run out of their battery energy. To keep comparisions fair, in case the execution of an algorithm completes before the other, its peak age still gets updated even though it is known that it would not be transmitting packets at future time instants. \par
%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.4]{figure/rr_vs_swc_weights_5_1_,1.eps}
%\centering
%\captionsetup{justification=justified, font={small,onehalfspacing}}
%\caption{Total weighted average peak age $\bar{\Delta}^p$ versus the ratio $\frac{t_s}{\mathbb{E}[T]}$ for an update system with $M=3$ sources.}
%%\vspace{-.1in}
%\label{peak_age_comp}
%\end{figure}
%\begin{table}[t]
%\footnotesize
% \centering
%\begin{tabular}{|l|l|l|l|}
%\hline
%Source & Weight & \begin{tabular}[c]{@{}l@{}}Initial battery \\ level (in mAh)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Target lifetime\\ (in hours)\end{tabular} \\ \hline
%Source 1 & 5 & 500 & 33.7 \\ \hline
%Source 2 & 1 & 1000 & 134.7 \\ \hline
%Source 3 & 0.1 & 1200 & 242.4 \\ \hline
%\end{tabular}
%\caption{Parameters of the heterogeneous sources.}
%\label{tab:my-table}
%\end{table}
%We first consider an information-update system with $M=3$ sources. We suppose that
%the transmission times are deterministic, i.e., $T_i= T=5$ ms for all $i$. Figure \ref{peak_age_comp} plots the total weighted average peak age $\bar{\Delta}^p$ versus the ratio $\frac{t_s}{T}$. The energy consumption rate for each source while it is transmitting, is equal to 24.75 mW. The weights $w_l$'s associated with various sources, their initial battery levels $B_l$'s, and target lifetimes $D_l$'s are as in Table \ref{tab:my-table}. As observed in Fig.~\ref{peak_age_comp} , the proposed sleep-wake algorithm outperforms the round robin for small values of $\frac{t_s}{\mathbb{E}[T]}$. This is because when the sensing time decreases, the probability of packet collision decreases. Moreover, our algorithm provides a near optimal trade-off between minimizing the AoI and energy consumption when the ratio $\frac{t_s}{T}$ is small. However, as we can see, the round robin algorithm outperforms our proposed sleep-wake algorithm for high values of $\frac{t_s}{T}$. This is reasonable, as increasing the sensing time leads to an increase in the probability of packet collision, and hence the age performance of the sleep-wake algorithm deteriorates. 



\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{figure/age_with_lower_bound_vs_energy_2.eps}
\centering
%\captionsetup{justification=justified, font={small,onehalfspacing}}
\captionsetup{justification=justified}
\caption{Total weighted average peak age $\bar{\Delta}^{\text{peak}}(\mathbf{r})$ versus the target energy efficiency $b$ for an update system with $M=10$ sources.}
%\caption{Total weighted average peak age $\bar{\Delta}^p$ versus the target lifetime $D$ for an update system with $M=10$ sources.}
%\vspace{-.1in}
\label{peak_age_comp_lower_bound}
\end{figure}

We now fix the value of $M$ at $10$ sources and the target energy efficiencies at the same value for all the sources, i.e., $b_l\equiv b$. We then vary the parameter $b$ and plot the resulting performances in Fig.~\ref{peak_age_comp_lower_bound}. We exclude simulations for $b< 0.1$ since the scheme of~\cite{chen2013life} is infeasible for Problem \textbf{1}. The age-optimal scheduler outperforms the rest of the schedulers and its performance is very close to the lower bound. Its performance is a decreasing function of $b$, and eventually settles at a constant value. This plot agrees with our analysis since from~\eqref{r_f_b_gr_1} we observe that there exists a value for $b$ after which our proposed solution value \textcolor{red}{is it $r^\star$??} is a function solely of weights $w_l$'s and $\beta^\star$, and not of $b$. Thus, unsurprisingly, the performance of the proposed scheduler saturates after this value of $b$. 










%We now consider an information-update system with $M=10$ sources. The target lifetimes of all the sources are taken to be the same, i.e., $D_l=D$ for all $l$. Figure \ref{peak_age_comp_lower_bound} plots the total weighted average peak age $\bar{\Delta}^{\text{peak}}$ versus the target lifetime $D$.
%% The mean of the packet transmission times is $\mathbb{E}[T]=5$ ms. 
%%The sensing time is $t_s=40~\mu$s. 
%%The energy consumption in a transmission mode is 24.75 mW.
% We consider homogeneous sources, where weight $w_l=1$, and initial battery level $B_l=300$ mAh, for all $l$. 
%The ``Lower bound” curve is generated from the lower bounds in \eqref{lower_bound_final_sumbi_ge1} and \eqref{lower_bound_72} in Appendix \ref{Appendix_A} that are constructed to solve Problem \textbf{1} and \textbf{2}. As we can observe, the total weighted average peak age increases as the target lifetime increases. This is because, as the target lifetime increases, our proposed sleep-wake algorithm reduces the packet transmission rate of the sources in order to meet the target lifetimes (or equivalently the energy constraints\textcolor{red}{equation number and is it battery?}), and hence AoI increases. We also observe that the total weighted average peak age of our proposed policy coincides with the lower bounds derived in\textcolor{red}{equation number?}. This is not surprising since the proposed sleep-wake algorithm is near age optimal in the regime when the ratio of the carrier sensing time to the mean transmission time ($\frac{t_s}{\mathbb{E}[T]}$) is small, which is .008 in this case. 
%%The plot also confirms that the bounds~\eqref{lower_bound_final_sumbi_ge1} and \eqref{lower_bound_72} are tight.

==> sections/Numerical_results_old.tex <==
\section{Numerical Results}\label{Simulations}
Throughout, we use ``Age-optimal scheduler'' to denote the sleep-wake scheduler with the sleep period paramters $r_l^{\star}$'s as in \eqref{r_f_b_gr_1}, which was shown to be near-optimal in Theorem \ref{thm_case_sum_bi_ge_1} and Theorem \ref{thm_case_sum_bi_le_1}. By ``Throughput-optimal scheduler'', we  refer to the sleep-wake algorithm of~\cite{chen2013life} that is known to achieve the optimal trade-off between the throughput and energy consumption. Also, we use ``Fixed-rate scheduler'' to denote the sleep-wake scheduler in which the sleep period parameters $r_l$'s are equal for all the sources, i.e., $r_l=k$ for all $l$ such that $k$ is chosen to satisfy the energy constraints in Problem \textbf{1}. Finally, the ``Lower bound'' curves are generated from the lower bounds in \eqref{lower_bound_sum_bi_ge_1} and \eqref{lower_bound_sum_bi_le_1}.

Unless stated otherwise, our setups are as follows: The average transmission time is $\mathbb{E}[T]=5$ ms. The weights $w_l$'s attached to different sources are generated by sampling from a uniform distribution in the interval $[0, 10]$. The target energy efficiencies $b_l$'s are randomly generated uniformly  within the range [0, 1]. 

%The energy consumption rate for each source while it is transmitting is equal to 24.75 mW. The initial battery levels and recharging rates are set to 
%$B_l\equiv 1200$ mAh, $R_l\equiv .22$ for all sources. The target lifetimes are chosen such that the target energy efficiencies $b_l$'s are randomly generated uniformly  within the range [0, 1]. \textcolor{red}{shouldnt it be other way around? }

\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{figure/comparison_life_add_no_users_10_vs_ration_2.eps}
\centering
%\captionsetup{justification=justified, font={small,onehalfspacing}}
\captionsetup{justification=justified}
\caption{Total weighted average peak age $\bar{\Delta}^{\text{peak}}(\mathbf{r})$ versus the ratio $\frac{t_s}{\mathbb{E}[T]}$ for an update system with $M=10$ sources.}
%\vspace{-.1in}
\label{peak_age_comp}
\end{figure}
\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{figure/comparison_life_add_vs_no_users.eps}
\centering
%\captionsetup{justification=justified, font={small,onehalfspacing}}
\captionsetup{justification=justified}
\caption{Total weighted average peak age $\bar{\Delta}^{\text{peak}}(\mathbf{r})$ versus the number of sources $M$.}
%\vspace{-.1in}
\label{peak_age_comp_num}
\end{figure}
Figures \ref{peak_age_comp} plot the total weighted average peak age $\bar{\Delta}^{\text{peak}}$ in \eqref{t_avg_peak_age} versus the ratio $\frac{t_s}{\mathbb{E}[T]}$.  We consider an information-update system with $M=10$ sources. As we can observe, the age-optimal scheduler outperforms the throughput-optimal and fixed-rate schedulers. This implies that what minimizes the throughput does not necessary minimize AoI and vice versa. Moreover, we can observe that the total weighted average peak age of the age-optimal scheduler converges to the lower bound as $t_s/\mathbb{E}[T]\to 0$. This agrees with our near-optimal results. Finally, we observe that the total weighted average peak age of all schedulers increases as the sensing time increases. This is reasonable, as increasing the sensing time leads to an increase in the probability of packet collisions, and hence the age performances of these schedulers deteriorate.



Figures  \ref{peak_age_comp_num} plot the total weighted average peak age $\bar{\Delta}^{\text{peak}}$ in \eqref{t_avg_peak_age} versus the number of sources $M$.   We set the sensing time to be $t_s=40~\mu$s. Again, we observe that the age-optimal scheduler outperforms the throughput-optimal and fixed-rate schedulers. Moreover, the total weighted average peak age of all schedulers increases with the number of sources, which is reasonable. Beside that, the gap between total weighted average peak age of age-optimal scheduler and the lower bound curve increase with the number of source. This is because the gap is a linearly increasing function of $C_1$ and $C_2$ in \eqref{eq23thm3_1} and \eqref{eq29thm3_3}, respectively, which increase with the number of sources. 

%As we can observe, our proposed sleep-wake algorithm outperforms the other two algorithms in both the cases. This is not surprising since the ``Life-add'' algorithm \textcolor{red}{of paper name..} was designed to maximize the throughput, and optimizing the throughput does not translate to optimizing the AoI. Moreover, in Figure \ref{peak_age_comp}, we observe that the total weighted average peak age for all algorithms increases as the sensing time increases. This is reasonable, as increasing the sensing time leads to an increase in the probability of packet collisions, and hence the age performances of these \textcolor{red}{is it all these algos?} algorithms deteriorate.

%while using the sleep-wake algorithm, we will set the rate parameters $r_l$ as in \eqref{r_f_b_gr_1}.
%We compare the performance of our proposed sleep-wake algorithm with the round robin \cite{li2013throughput,hsu2017scheduling,kadota2016minimizing,kadota2016minimizing_journal,jiang2018timely}. Under the round robin algorithm sources take turns in order to transmit their update packet. Thus, once a source obtains channel access, it transmits until its battery dies out. The execution of an algorithm is completed when all the sources run out of their battery energy. To keep comparisions fair, in case the execution of an algorithm completes before the other, its peak age still gets updated even though it is known that it would not be transmitting packets at future time instants. \par
%\begin{figure}[t]
%\centering
%\includegraphics[scale=0.4]{figure/rr_vs_swc_weights_5_1_,1.eps}
%\centering
%\captionsetup{justification=justified, font={small,onehalfspacing}}
%\caption{Total weighted average peak age $\bar{\Delta}^p$ versus the ratio $\frac{t_s}{\mathbb{E}[T]}$ for an update system with $M=3$ sources.}
%%\vspace{-.1in}
%\label{peak_age_comp}
%\end{figure}
%\begin{table}[t]
%\footnotesize
% \centering
%\begin{tabular}{|l|l|l|l|}
%\hline
%Source & Weight & \begin{tabular}[c]{@{}l@{}}Initial battery \\ level (in mAh)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Target lifetime\\ (in hours)\end{tabular} \\ \hline
%Source 1 & 5 & 500 & 33.7 \\ \hline
%Source 2 & 1 & 1000 & 134.7 \\ \hline
%Source 3 & 0.1 & 1200 & 242.4 \\ \hline
%\end{tabular}
%\caption{Parameters of the heterogeneous sources.}
%\label{tab:my-table}
%\end{table}
%We first consider an information-update system with $M=3$ sources. We suppose that
%the transmission times are deterministic, i.e., $T_i= T=5$ ms for all $i$. Figure \ref{peak_age_comp} plots the total weighted average peak age $\bar{\Delta}^p$ versus the ratio $\frac{t_s}{T}$. The energy consumption rate for each source while it is transmitting, is equal to 24.75 mW. The weights $w_l$'s associated with various sources, their initial battery levels $B_l$'s, and target lifetimes $D_l$'s are as in Table \ref{tab:my-table}. As observed in Fig.~\ref{peak_age_comp} , the proposed sleep-wake algorithm outperforms the round robin for small values of $\frac{t_s}{\mathbb{E}[T]}$. This is because when the sensing time decreases, the probability of packet collision decreases. Moreover, our algorithm provides a near optimal trade-off between minimizing the AoI and energy consumption when the ratio $\frac{t_s}{T}$ is small. However, as we can see, the round robin algorithm outperforms our proposed sleep-wake algorithm for high values of $\frac{t_s}{T}$. This is reasonable, as increasing the sensing time leads to an increase in the probability of packet collision, and hence the age performance of the sleep-wake algorithm deteriorates. 



\begin{figure}[t]
\centering
\includegraphics[scale=0.4]{figure/age_with_lower_bound_vs_energy_2.eps}
\centering
%\captionsetup{justification=justified, font={small,onehalfspacing}}
\captionsetup{justification=justified}
\caption{Total weighted average peak age $\bar{\Delta}^{\text{peak}}(\mathbf{r})$ versus the target energy efficiency $b$ for an update system with $M=10$ sources.}
%\caption{Total weighted average peak age $\bar{\Delta}^p$ versus the target lifetime $D$ for an update system with $M=10$ sources.}
%\vspace{-.1in}
\label{peak_age_comp_lower_bound}
\end{figure}
In Figure \ref{peak_age_comp_lower_bound}, we consider an information-update system with $M=10$ sources, where   the target energy efficiency of all sources are taken to be the same, i.e., $b_l=b$ for all $l$. Figure \ref{peak_age_comp_lower_bound} plots the total weighted average peak age $\bar{\Delta}^{\text{peak}}$ in \eqref{t_avg_peak_age} versus the target energy efficiency $b$. We can observe that, we start our simulation from the point $b=0.1$. This is because, in enegry-scarce regime, i.e., when $\sum_{i=1}^Mb_i<1$, the sleeping period parameters that are proposed in \cite{chen2013life} are not feasible for Problem \textbf{1}, and hence we cannot compare our proposed scheduler with the throughput-optimal scheduler in this case. We can observe that the age-optimal scheduler outperforms the throughput-optimal and fixed-rate schedulers and its total weighted average peak age comes close to the lower bound curve. Moreover, as the target efficiency $b$ increases, the total weighted average peak age of age-optimal scheduler decreases and then saturates. To understand this behavior, let us recall our proposed solution in \eqref{r_f_b_gr_1}. We can observe that there exists a value for $b$ after which our proposed solution value depends only on the weights $w_l$'s and $\beta^\star$ and does not depend on $b$. That is way, the age performance of our proposed scheduler saturates after this point. 










%We now consider an information-update system with $M=10$ sources. The target lifetimes of all the sources are taken to be the same, i.e., $D_l=D$ for all $l$. Figure \ref{peak_age_comp_lower_bound} plots the total weighted average peak age $\bar{\Delta}^{\text{peak}}$ versus the target lifetime $D$.
%% The mean of the packet transmission times is $\mathbb{E}[T]=5$ ms. 
%%The sensing time is $t_s=40~\mu$s. 
%%The energy consumption in a transmission mode is 24.75 mW.
% We consider homogeneous sources, where weight $w_l=1$, and initial battery level $B_l=300$ mAh, for all $l$. 
%The ``Lower bound” curve is generated from the lower bounds in \eqref{lower_bound_final_sumbi_ge1} and \eqref{lower_bound_72} in Appendix \ref{Appendix_A} that are constructed to solve Problem \textbf{1} and \textbf{2}. As we can observe, the total weighted average peak age increases as the target lifetime increases. This is because, as the target lifetime increases, our proposed sleep-wake algorithm reduces the packet transmission rate of the sources in order to meet the target lifetimes (or equivalently the energy constraints\textcolor{red}{equation number and is it battery?}), and hence AoI increases. We also observe that the total weighted average peak age of our proposed policy coincides with the lower bounds derived in\textcolor{red}{equation number?}. This is not surprising since the proposed sleep-wake algorithm is near age optimal in the regime when the ratio of the carrier sensing time to the mean transmission time ($\frac{t_s}{\mathbb{E}[T]}$) is small, which is .008 in this case. 
%%The plot also confirms that the bounds~\eqref{lower_bound_final_sumbi_ge1} and \eqref{lower_bound_72} are tight.

==> sections/learning_backup_before_dividing.tex <==
\section{Analysis of Learning Algorithm}\label{sec:learn_proof}
We begin by showing that the quantity $s(t)$ can be taken to be the system state \slash sufficient statistics~\cite{striebel1965sufficient} in order to describe the sampled process. In what follows, we let $\cS := \bR_{+}\times \{0,1\}$. Denote by $\te :=  \int_{y=0}^{T_{\max}} f(y) dy$ the mean transmission time of a packet of any source, i.e., we use the abbreviation $\te = \bE\left[T\right]$. The proof of the following result is omitted for brevity.
%Let the waiting time employed by a source be an exponential r.v. with mean value $1$. 
\begin{lemma}\label{lemma:suff_stat}
Consider the system in which $M$ sources share a channel, and utilize the sleep period paremeters as $u(t)\equiv \br$ in order to modulate the sleep durations of sources. We then have that
\begin{align}\label{def:kernel_exist}
\bP\left(  s(t+1) \in A \big|  \cF_t \right) = K(s(t),u(t),A;f), \forall A \in \cS^{M},
\end{align}
where $\cF_t$ denotes the sigma-algebra generated by all the random variables until the $t$-th discrete sampling instant. % $K: \cS^{M} \times \bR^{M}_{+}\mapsto [0,1]$ is a measurable function, and $f$ is the probability density function of the transmission time. 
The function $K$ is the kernel~\cite{nummelin2004general} associated with the controlled transition probabilities of the process $s(t)$, 
\begin{align}\label{def:kernel}
K: \cS^{M} \times \cB(\bR^{M}) \mapsto [0,1],
\end{align}
thus, $K(s,r,A;f)$ is the probability with which the state at time $t+1$ belongs to the set $A$, given that the state at time $t$ is equal to $s$, and the vector comprising of sleep period parameters at time $t$ is equal to $r$. Note that the kernel is parametrized by the density function of transmission time $f$.
\end{lemma}
From now onwards, we will work exclusively with the discrete-time system obtained by sampling the original continuous-time system. Consider the operation over a time horizon of $H$ discrete time-steps, and let $K_{l}$ denote the (random) number of packets delivered to source $l$ until time $H$. The cumulative cost incurred is given by
\begin{align}\label{def:peak_cost}
C(H) := \sum_{l=1}^{M}  \sum_{i=1}^{K_l}  \Delta^{\text{peak} }_{l,i},
\end{align}
where $\Delta^{\text{peak}}_{l,i}$ denotes the $i$-th peak age of source $l$. We now show that in order to minimize the expected value of $C(H)$, it suffices to design controllers that ``work directly'' with the sampled system. Thus, the quantity $s(t)$ as described in~\eqref{def:st} serves as a sufficient statistic for the purpose of optimizing the expectation of cumulative peak age~\cite{striebel1965sufficient}. We also show that this objective can be posed as a Markov decision process~\cite{puterman2005markov}.
\begin{lemma}\label{lemma:equiv_problem}
Let $s(t), t=1,2,\ldots,$ be the sampled controlled Markov process. There exists a function $g: \cS^{M} \mapsto \bR$ so that $\bE\left[C(H)\right]$~\eqref{def:peak_cost} is given by $\bE \left[\sum\limits_{t=1}^{H} g(s(t))\right]$.  
\end{lemma}
\begin{proof}
Consider the cumulative peak-age cost~\eqref{def:peak_cost} in which the $l$-th source incurs a penalty of $\Delta^{\text{peak}}_{l,i}$ upon delivery of the $i$-th packet. Let this delivery occur at the end of the $t$-th discrete time-slot (note that this time $t$ is random). Let us denote by $a^{\text{peak}}_{l}(t)$ the peak age of source $l$ during the (continuous) time interval (in the non-discretized system) corresponding to the discrete time slots $t-1$ and $t$. We could (instead of charging a penalty of $\Delta^{\text{peak}}_{l,i}$ units at the end of $t$-th slot) charge the quantity $\bE\left\{a^{peak}(t)| s(t-1),u(t-1)\right\}$ at the discrete time instant $t-1$. For sources $k\neq l$ that are not transmitting between $t-1$ and $t$, and have $m_k(t-1)=0$, we let $g(s(t-1))=0$. It then follows from the law of the iterated expectations~\cite{billingsley2008probability} that the expected cost of the system under this modified cost function remains the same as that of the original system. This completes the proof. 
\end{proof}  

\subsection{System Description}
In what follows, we let $r_l(t) \in \bR_{+}$ denote the sleep period parameter for source $l$ at time $t$, and denote $\br(t):=\left(r_1(t),r_2(t),\ldots,r_M(t)\right)$. The controller that chooses $\br(t)$ does not know the density function $f$ of the packet transmission time, and has to adaptively choose the sleeping period paremeter $\br(t)$ so as to minimize the operating cost as measured by the expected value of peak age, i.e., the quantity 
\begin{align}\label{def:cost}
\bE \left(\sum_{t=1}^{H-1}~g(\bs(t)) \right),
\end{align}
where the function $g$ is as in Lemma~\ref{lemma:equiv_problem}. 

Let $\cF^{(d)}_t$ denote the sigma-algebra generated by the random variables $\{\bs(i)\}_{i=1}^{t}, \{\br(i)\}_{i=1}^{t-1}$ (the super-script $d$ denotes the fact that we are working with discretized system). A learning policy is a collection of maps $\cF^{(d)}_t\mapsto \br(t), t=1,2,\ldots,H$. The performance of a learning policy is measured by its regret $R(H)$, which is defined as follows,
\begin{align}\label{def:regret}
R(H) := \sum_{t=1}^{H}  g(\bs(t)) - H \bar{\Delta}^{\text{w-peak}}(\mathbf{r}^{\star}),
\end{align}
where $\bar{\Delta}^{\text{w-peak}}(\mathbf{r}^{\star})$ is the optimal performance when the true system parameter is known and hence scheduler can implement the optimal rate vector. Since the optimal rate depends upon the probability density function $f(\cdot)$ only through its mean $\bE\left[T\right]$, we also denote it by $\br\ust_{\te}$. % We denote this optimal rate vector as $r\ust(f)$. 
\subsection{Preliminary Results}\label{sec:jmls}
\begin{comment}
\textcolor{red}{Cite some book here..} We let $V_{\te,r}(\cdot):\bR^{N}\mapsto \bR$ denote the ``differential cost function'' for the system in which the mean transmission time is equal to $\theta$, and the control policy uses $u(t)\equiv r$. We also let $J_{\te,r}$ be the corresponding operating cost. Thus,
\begin{align}\label{eq:cost_diff}
J_{\te,r} + V_{\te,r}(x) = g(x) +  \bE V_{\te,r}( f(x(t),w(t);\te,r) ), \forall x\in \bR^{N}_{+}.
\end{align}
\end{comment}


\emph{Notation}: For two integers $n_1,n_2\in \bZ$, we let $[x,y]:= \left\{x,x+1,\ldots,y\right\}$. For a set of r.v. s $\cX$, we let $\cF(\cX)$ denote the smallest sigma-algebra with respect to which each r.v. in $\cX$ is measurable. For functions $f(x),g(x)$, we say $f(x)=O(g(x))$ if $\lim_{x\to\infty} f(x)\slash g(x)=1$. For a set $\cX$, we let $\cX^{c}$ denote its complement. For an event $\cX$, we let $\id(\cX)$ denote its indicator random variable. For a set $\cX$, we let $\cB(\cX)$ denote the sigma-algebra of Borel sets of $\cX$.\par

We begin by stating some definitions associated with Markov Chains on \emph{General State-Spaces}. Though these can be found in standard textbooks on General State-Space Markov Chains such as~\cite{meyn2012markov,nummelin2004general}, we include them here in order to make the paper self-contained.  

Let us now fix the controls at $\br(t)\equiv \br$, and consider the resulting discrete-time Markov chain $s(t)\in \cS^{M}$. If $A$ is a Borel set, we let $P^{n}(s,A)$ denote the probability of the event $s(n)\in A$, given that $s(0) = x$.
\begin{definition}(Small Set)\label{def:small}
A set $C\in  \cB(\cS^{M})$ is called $\nu_m$ small if for all $x\in C$ we have that 
\begin{align*}
P^{m}(x,A) \ge \nu_m(A),~\forall  A\in \cB(\cX),
\end{align*}
for some non-trivial measure $\nu_m(\cdot)$ and some $m\in \bN$. 
\end{definition}

\begin{definition}(Petite Set)
Let $q = \{q_n\}_{n\in \bN}$ be a probability distribution on $\bN$. A set $C\in  \cB(\cS^{M})$, and a non-trivial sub-probability measure $\nu$ are called petite if we have that
\begin{align*}
\sum_{n\in \bN} q_n P^{n}(x,A)\ge \nu_{q}(A), \forall A\in \cB(\cS^{M}),\forall x\in C. 
\end{align*}
\end{definition}

\begin{definition}(Strong Aperiodicity)
If there exists a $\nu_1$ small set $C$ such that we have $\nu_1(C)>0$, then the chain $s(t)$ is strongly aperiodic.  
\end{definition}

We begin by deriving the following preliminary results about the Markov process $s(t)$.
\begin{lemma}\label{lemma:petite}
Consider the multi-source wireless network operating under the controls $\br(t)\equiv \br$, and assume that the sensing time $t_s$ is sufficiently small, i.e., it satisfies $t_s<1$. Consider the associated process $s(t),~t=1,2,\ldots,$. We then have the following:\\
\begin{enumerate}
\item Define
\begin{align*}
e_i := (M-i)\epsilon, \mbox{ and } m_i = 0, \forall i \in [N], 
\end{align*}
where $\epsilon>0$ is chosen to be sufficiently small. Consider the set 
\begin{align}\label{def:set_C}
C:= \otimes_{i=1}^{N} \left[ [ (M-i), (M-i) + e_i ] \times \left\{m_i\right\} \right].
\end{align}
The set $C$ is small for the process $s(t)$.
\item For the process $s(t)$, each compact set is petite.
\item The process $s(t)$ is strongly aperiodic.
\end{enumerate}
\end{lemma}
\begin{proof}
\par 
\begin{enumerate}
\item Consider $s(0)\in C$. It follows that at time $t=0$, all the sources are sleeping. Consider the following set denoted $C^{\prime}$: Sources $1$ and $2$ wake up within $t_s$ time duration of each other, while the other sources wake up much later than these two. Consequently, there is a collision between Source $1$ and Source $2$, and hence at time $t=1$ these two sources enter into sleep mode, so that at time $t=1$ all the sources are asleep. Also assume that the cumulative time elapsed for this event to occur is approximately equal to $t_s + \delta$, where $\delta>0$ is a sufficiently small parameter. The probability of the event $\left\{s(1)\in C^{\prime}\right\}$ can be lower bounded as follows 
\begin{align*}
\bP(s(1)\in C^{\prime} )\ge \left( r_1  \int_{\delta}^{\delta+\epsilon} \exp(-r_1 x) dx\right) t_s  r_2  \exp(-r_2 (\delta+\epsilon)) \left[\Pi_{i=3}^{N}  \int_{\delta+\epsilon}^{\infty} r_i \exp(-r_i x) dx\right].
\end{align*}
Since the above lower-bound on the probability of ``reaching $C^{\prime}$'' is true for all $x(0)\in C$, it follows from Definition~\ref{def:small} that the set $C$ is small.
\item Consider the process $s(t)$ starting in state $s(0)$, and let the age vector $a(0)$ satisfy $\sum_{i=1}^{N}  a_i(0)\le K$ where $K>0$, so that $s(0)$ belongs to a compact set.
We will derive a lower bound on the probability of the event $\left\{s(N)\in C\right\}$, where $C$ is as in~\eqref{def:set_C}. This will prove (ii) since we have already shown in (i) that the set $C$ is small. Consider the following sample path: at each time $i\in [1,M]$, we have that source $i$ successfully transmits a packet, and moreover the age of the packet received is approximately equal to $1$. We will derive a lower-bound on the probability of this event. In the following discussion we use $b>0$ and $\eta \in \left( 0, 1-t_s-b\right)$, where $\eta$ denotes the time when Source $1$ wakes up. Since the counter of the $i$-th source has a probability density equal to $r_i e^{-r_i x}$, the probability that during the $i$-th slot source $i$ gets channel access is lower bounded by $(1- \exp(-\eta r_i))\Pi_{j\neq i} e^{-r_j}  $; while the probability that the age of its delivered packet is around $1$, given that it wakes up at $\eta$, is lower bounded by $\int_{0}^{b} f(y)dy$. Thus, the probability of this sample path is lower bounded by
\begin{align*}
\Pi_{i=1}^{N} (1- \exp(-\eta r_i))\Pi_{j\neq i} e^{-r_j}   \int_{0}^{b} f(y)dy.
\end{align*}
This concludes the proof since along this sample path we have that $s(N)\in C$.
\item It follows from the discussion on page 121 of~\cite{meyn2012markov} that in order to prove the claim it suffices to show that the volume of the set $C\cap C^{\prime}$ is greater than $0$. However, this condition holds true if the parameter $\delta$ in (i) above has been chosen so as to satisfy $t_s + \delta< \epsilon$. 
\end{enumerate}
\end{proof}

We now show that the process $x(t)$ has a certain ``mixing property''.
For a measure $\mu$ and a function $f$, we define $\|\mu\|_f :=  \int f(x) d\mu(x) $.
\begin{lemma}[Geometric Ergodicity]\label{lemma:geometric}
Consider the Markov process $s(t),~t=1,2,\ldots,$ associated with the network in which the controller utilizes $\br(t)\equiv \br $. The Markov process $s(t)$ has an invariant probability measure, which we denote as $\pi(\infty,\br)$. Moreover, 
\begin{align}\label{ineq:geometric}
&\int \left(\|y\|_1 +1\right)  d\left( P^{n}(x,\cdot) - \pi(\infty,r)\right)(y) \notag \\
&\le  R\left( \|x(0)\|_1 +1 \right) \rho^{n}, n\in \bN,
\end{align}
where $R>0$.
%where $f(x)= $, \textcolor{red}{and $R = ?\cdots $ directly substitute for $R$}. 
\end{lemma}
\begin{proof}
It follows from Theorem 6.3 of~\cite{meyn2012markov} that it suffices to show that the following holds true when $\|s(t+1)\|_1 $ is sufficiently large enough
\begin{align}\label{eq:cond_geometric}
\bE\left( \|s(t+1)\|_1 | \cF_{t} \right)  \le     \lambda \|s(t)\|_1 + L,
\end{align} 
where $\lambda<1$. Note that each source gets to transmit with a probability at least $\min_l \alpha_{l}$, and also the expected value of the inter-sampling time is upper-bounded by $\max\left\{\bE [T],\frac{\bE[T]}{\sum_{i=1}^Mr_i}+t_s\right\}$. It then follows that~\eqref{eq:cond_geometric} holds true with $\lambda$ set equal to $\min_l \alpha_{l}$, and $L$ equal to $\max\left\{\bE [T],\frac{\bE[T]}{\sum_{i=1}^Mr_i}+t_s\right\}$.
\begin{comment} commenting this part out after discussion with Ahmed
We consider the following two possibilities:\\
(i) At time $t$, the source with the largest value of age $\Delta_l(t)$ gets access to the channel within $1 + t_s$ time, and then transmits a packet. Since source $l$ gets access within $1$ units of time, w.p. atleast $\min_{l\in [1,M]}  (1-e^{-r_l}) \Pi_{i\neq l} e^{-r_i}$; we have that this event occurs with atleast this probability. Since the time taken to transmit packet is bounded by $1$, in the case of this event, the age of source $l$ is bounded by $B+1+t_s$.\\
(ii) On the complement of (i), we can bound (in distribution) the time taken for the channel access decision, by an individual source's  
we upper-bound the expected cumulative increase in age as follows. We add the time duration until the next sampling instant to the age of all sources. Since the time until next sampling time can be upper-bounded by an exponentially distributed random variable with parameter $\min_i r_i$, we have that  the expected increase in cumulative age of all sources is upper-bounded by $\frac{N}{\min_i  r_i}$.

Combining (i), (ii) above, we obtain that  
Upon combining (i) and (ii) above, we conclude that~\eqref{eq:cond_geometric} holds with 
\begin{align*}
\lambda =  1- \frac{\min_{i\in [1,N]}  (1-e^{-r_i}) \Pi_{j\neq i} e^{-r_j}   \left(1-e^{-1}\right)}{N},
\end{align*}
and
\begin{align*}
L = \frac{N}{\min_{i\in [1,N]}}.
\end{align*}
\end{comment}
\end{proof}

\begin{lemma}(Differential Cost Function)\label{lemma:diff_co}
Consider the process $s(t),~t=1,2,\ldots,$ that describes the evolution of the network in which the controller utilizes $u(t)\equiv \br$. Then, there exists a function $V: \cS^{M}\mapsto \bR $ that satisfies
\begin{align}\label{eq:diff_cost}
V(x) + \int  g(x) d\pi(\infty,\br) = g(x) + \int  K(x,r,y;f) V(y)dy.
\end{align}
Moreover, the function $V$ satisfies the following,
\begin{align}
V(x) \le \frac{R}{1-\rho} \left( \|\Delta(0)\|_1 +1 \right). 
\end{align}
\end{lemma}
\begin{proof}
We have shown in Lemma~\ref{lemma:geometric} that the process $s(t)$ is geometrically ergodic. Hence, it follows from Theorem 7.5.10 of~\cite{hernandez2012further} that there exists a function $V(\cdot)$ that satisfies~\eqref{eq:diff_cost}, and moreover it is given as follows, 
\begin{align*}
V(x) = \sum_{t=1}^{\infty} \left[\bE_{x}\left(g(x(t))\right) -  \int_{\cS^{M}}   g(y)d \pi(\infty,\br)\right], x\in \cS.
\end{align*}
Substituting the geometric bound~\eqref{ineq:geometric} into the above, we obtain the following
\begin{align*}
V(x) &= \sum_{t=1}^{\infty} \left[\bE_{x}~ g(x(t)) -  \int_{\cS^{M}}   g(y)d \pi(\infty,\br)\right]\\
&\le \sum_{t=1}^{\infty} \Big| \bE_{x}~ g(x(t)) -  \int_{\cS^{M}} g(y)d \pi(\infty,\br)\Big|\\
&\le R\left( \|x(0)\|_1 +1 \right) \sum_{t=1}^{\infty} \rho^{t}\\
&= \frac{R\left( \|x(0)\|_1 +1 \right) }{1-\rho},
\end{align*}
where $\rho<1$. 
\begin{comment}
Define
\begin{align*}
\tilde{V}_n(x):= \sum_{t=1}^{n} \left[\bE_{x}~ g(x(t)) -  \int   g(x)d \pi(\infty,r)\right], x\in \cX.
\end{align*}
For $m<n$, we have that 
\begin{align*}
| V_n(x) - V_m(x) | &=  \Bigg|\sum_{t=m}^{n} \left[\bE_{x}~ g(x(t)) -  \int   g(x)d \pi(\infty,r)\right] \Bigg| \\
&\le \sum_{t=m}^{n} \Big|\bE_{x}~ g(x(t)) -  \int   g(x)d \pi(\infty,r)  \Big|  \\
&= \sum_{t=m}^{n} \Big|\int g(x) dP^{n}(x,\cdot)  -  \int   g(x)d \pi(\infty,r)  \Big|  \\
&\le \sum_{t=m}^{n} \Big|\int g(x) dP^{n}(x,\cdot)  -  \int   g(x)d \pi(\infty,r)  \Big|  \\
& \le \frac{R(x+1) \rho^{m} }{1-\rho},
\end{align*}
where the last inequality follows from Lemma~\ref{lemma:geometric}. This shows that $V_n(x), n\in \bN$ is Cauchy, and hence converges. Let $V(x)$ be the convergent value. Now we have,
\begin{align*}
\tilde{V}_{n+1}(x) = g(x) -  \int g(x) d \pi(\infty,r)   + \bE \tilde{V}_{n} \left(f(x,u,w)\right),  
\end{align*}
which yields,
\begin{align*}
\tilde{V}_{n+1}(x) +  \int g(x) d \pi(\infty,r)  = g(x)   + \bE \tilde{V}_{n} \left(f(x,u,w)\right).
\end{align*}
Since $\tilde{V}$
\end{comment}

\end{proof}

\begin{lemma}\label{lemma:convergence}
\begin{enumerate}[(i)]
\item We have that the function $\br\ust_{\te}: \Theta \mapsto \bR^{M}_{+}$ that maps the mean transmission time $\te$ to the optimal sleep period parameter, is a continuous function of $\theta$. Similarly, the average peak age is a continuous function of $\br$, i.e.,
\begin{align*}
\lim_{\br\to \br\ust_{\te}}\lim_{H\to\infty}\frac{1}{H} \sum_{t=1}^{H} \bE_{\br} \left[g(s(t))\right]  \to \lim_{H\to\infty}\frac{1}{H} \sum_{t=1}^{H} \bE_{\br\ust_{\te}} \left[g(s(t))\right], 
\end{align*}
where the sub-script $\br$ in the expectation $\bE_{\br}$ above refers to the fact that the averaging is performed w.r.t. the measure induced by the policy that uses sleep rates equal to $\br$.
\item The cumulative peak-age $\bar{\Delta}^{w-peak}(\br)$ is locally Lipschitz continuous function of $\br$. Thus,
\begin{align*}
|\bar{\Delta}^{w-peak}(\br\ust_{\te};\te) - \bar{\Delta}^{w-peak}(\br;\te) | \le L_{1}  \|\br\ust_{\te} - \br\|,
\end{align*}
whenever $\|\br\ust_{\te} - \br \|$ is sufficiently small, and where the Lipschitz constant at  sleep period parameter $\br$ is given by 
\begin{align*}
L_{1} := \max_{i\in [M]} \frac{\partial \bar{\Delta}^{w-peak}}{\partial r_i}(\br).
\end{align*}
Similarly, the optimal sleep period parameter is a locally Lipschitz function of $\te$, so that we have,
\begin{align*}
\|\br\ust_{\te_1} - \br\ust_{\te_2} \|\le L_{2}  |\te_1 - \te_2|, L_2>0,
\end{align*}
whenever $ |\te_1 - \te_2|$ is sufficiently small.
\end{enumerate}
\end{lemma}
\begin{proof}
Continuity of the functions under discussion is immediate from the relations \eqref{r_f_b_gr_1}, \eqref{x*}, \eqref{condition_beta}, \eqref{condition_x*_beta*}, \eqref{feasible_factor}, \eqref{feas_fact_eq27}. 
\begin{comment}
To show (ii), we use Theorem~1 of~\cite{karr1975weak}; from which it follows that it suffices to show the following (\textcolor{red}{should it be $A\in \cB(\cS^{M})$? })
\begin{align*}
\sup_{x\in C} | K(x,\br,A;f) - K(x,\br\ust_{\te},A;f) | \to 0,\forall A\in \cS^{M},
\end{align*}  
where $K(x,r,\cdot;f)$ is the one-step probability transition kernel when the sleep period parameter is equal to $\br$, and $C$ is a compact subset of $\cS^{M}$. 
\end{comment}
To prove the statement about Lipschitz continuity, it suffices to show that the average peak age is a Lipschitz continuous function of $\br$, and the optimal rate $\br\ust_{\te}$ is Lipschitz continuous function of $\te$. To prove this, it suffices to show that the average peak age is a continuously differentiable function of $\br$, and also $\br\ust_{\te}$ is a continuously differentiable function of $\te$ (see~\cite{hunter} for more details). The continuously differentiable property is evident from the relations~\eqref{t_avg_peak_age},~\eqref{r_f_b_gr_1}-\eqref{condition_beta} and~\eqref{condition_x*_beta*}-\eqref{feas_fact_eq27}. This completes the proof.
\end{proof}
\subsection{Learning Algorithm}
Let $\hat{\theta}(t)$~denote the empirical estimate of $\theta$ at time $t$, i.e., 
\begin{align}\label{def:point_est}
\hat{\theta}(t) &:=\frac{\sum_{i=1}^{t} T(i) col(i)}{N(t)\vee 1},\\
N(t) :&= \sum_{i=1}^{t} col(i)
\end{align}
where $T(i)\in \left[0,T_{\max}\right]$ is the time taken to deliver packet at time $i$; while $col(i)$ denotes the collision process that assumes value $1$ if there was no collision at time $i$, and is $0$ otherwise. We also let $ca_{l}(i)=1$ if source $l$ gets channel access at time $i$, while $ca_{l}(i)$ is $0$ otherwise. 

The learning rule operates in episodes. We let $\tau_k$ be the start time of the $k$-th episode, and let $\cE_k := [\tau_k,\tau_{k+1}-1]$ be the time-slots comprising $k$-th episode so that its duration is $\tau_{k+1} - \tau_k$ time-slots. Let $k(t)$ be the index of the current episode, and $\te(t)$ be the empirical estimate at the beginning of the current episode, 
\begin{align}\label{def:ucb_problem}
k(t) :&= \max\left\{ k: \tau_k \le t  \right\},\\
\te(t) :&= \hat{\theta}(\tau_{k(t)}). 
\end{align}
The learning rule that we propose, implements a single stationary controller within each single episode: this controller makes decisions only on the basis of the state $s(t)$ and the estimate $\te(\tau_k)$ obtained at the beginning of the current ongoing episode $k(t)$. It chooses the sleeping period parameter as $\br(t)= \br\ust_{\te(t)}$, i.e., it utilizes the rate vector that is optimal in the event the true value of the mean transmission time is the same as the empirical estimate obtained at the beginning of the current episode. Thus, $\br(t)= \br^{\star}_{\theta(\tau_k)}$ for $t\in\left[\tau_k,\tau_{k+1}-1\right]$. We summarize our learning rule in Algorithm~\ref{algo:ucb}. 
\begin{assumption}
With a high probability, say greater than $1-\delta$, where $\delta>0$ is a small constant, the state value $s(\tau_k)$ at the beginning of each episode $k$ belongs to a compact set $\cK:= \left\{ x\in \cS^{M}: \|x\|_1 \le K_1  \right\}$.  
\end{assumption}
The above is not a restrictive assumption, since the scheduler can always ensure that towards the end of each episode, each source receives sufficient amount of service in order to ensure this condition. We now make few assumptions regarding the set $\Theta$ of ``allowable parameters''.

\begin{assumption}\label{assum:2}
We have 
\begin{align*}
\limsup_{H\to\infty} \frac{1}{H} \sum_{t=1}^{H} \bE_{\br^{\star}_{\te}}\left(g(x(t))\right) & \le K_2 <\infty,\\
\inf_{\te \in \Theta,l\in [M]} \bP\left( ca_{l}(t)=1| u(t)= \br^{\star}_{\te} \right) & >0.
\end{align*}
We denote
\begin{align}\label{def:cmin}
p_{\min} := \inf_{\te \in \Theta,l\in [M]} \bP\left( ca_{l}(t)=1| \br(t)= \br^{\star}_{\te} \right). 
\end{align}

\end{assumption}

 \begin{algorithm}
 \begin{algorithmic}[1]
 \renewcommand{\algorithmicrequire}{\textbf{Input:}}
 \REQUIRE $N,\gamma>2$\\
 Set $\hat{\theta}(1)=.5$.
  \FOR {$t=1,2,\ldots$} 
  \IF {$t = \tau_k$}
  \STATE Calculate $\hat{\theta}(t)$ as in~\eqref{def:point_est} and $\theta(t)$ by solving~\eqref{def:ucb_problem}. \\
  \ELSE 
  \STATE $\hat{\theta}(t)=\hat{\theta}(t-1)$
  \ENDIF\\
  Calculate $u(t)$ based on current estimate $\theta(t)$
  \ENDFOR
   \caption{Learning for AoI Optimization}\label{algo:ucb}
 \end{algorithmic} 
\end{algorithm}
%We note the following. During each discrete time-slot, each source $i$ gets to transmit with a certain probability, that depends upon $\theta\ust$ and $u(t)$. We perform analysis under the following assumption.
%\begin{assumption}
%The set $\Theta$, satisfies the following
%\begin{align}
%\sum_i \bP\left( i \mbox{ gets to transmits } |  u(t)=r^{\star}_{\theta}  \right) > \alpha >0, \forall \theta\in \Theta. 
%\end{align}
%\end{assumption}

\subsection{Regret Analysis}
We begin by deriving some concentration results for the estimate $\hat{\theta}(t)$ around the true mean.

\emph{Bounds on the Estimation Error}: 
Let $\cC(t)$ be the confidence interval associated with the estimate $\hat{\theta}(t)$, i.e., 
\begin{align}\label{def:ucb_ci} 
\cC(t) := \left\{ \theta :  |\theta -\hat{\theta}(t) | \le  \xi(t), \theta >0 \right\},
\end{align} 
where
\begin{align*}
\xi(t) : =  T_{\max}\sqrt{\frac{2 \log\left(t^{\gamma}\right)}{N(t)}}, t\in [1,H],
\end{align*}
$\gamma>2$ is a source-specified constant, $N(t)$ is the total number of packet deliveries until $t$, and $T_{\max}$ is the maximum possible transmission time. We begin by showing that with a high probability, the true parameter $\theta$ lies within the confidence ball $\cC(t)$ at all the times.
\begin{lemma}\label{lemma:g1}
Define %(\textcolor{green}{Good Sets 1})
\begin{align*}
\cG_1(t) := \left\{ \omega: \theta\ust \in \cC(t)\right\},
\end{align*}
where $\cC(t)$ is as in~\eqref{def:ucb_ci}. We then have that
\begin{align*}
\bP\left( \cG^{c}_{1}(t)  \right) \le \frac{1}{t^{\gamma -1}}.
\end{align*}
\end{lemma}
\begin{proof}
Fix a positive integer $n$, and consider the empirical estimate $\hat{\te}$ obtained after $n$ samples $T(1),T(2),\ldots,T(n)$ of the service times. It follows from Azuma-Hoeffding's inequality~\cite{hoeffding1994probability} that
\begin{align*}
\bP\left(  |\hat{\te} -  \te^{\star}  | >  x  \right)  \le \exp\left(-\frac{n x^{2}}{2 T_{\max}^{2} }      \right).
\end{align*}
By using $x = T_{\max}\sqrt{ \frac{2\log \left( t^{\gamma}\right) }{n}    }$ in the above, we obtain,
\begin{align*}
\bP\left(  |\hat{\te} -  \te^{\star}  | >   \sqrt{ \frac{\log t^{\gamma} }{n}    }  \right) & \le \exp\left(-\log t^{\gamma}       \right)  \\
&=  \frac{1}{t^{\gamma}}.
\end{align*}
Since the total number of samples $n$ can assume values in the set $[t]$, the proof then follows by using union bound on $n$.
\end{proof}
\vspace{.5cm}

\begin{lemma}\label{lemma:g2}
Fix a $\delta_1 \in \left(0, p_{\min}\right)$, where $p_{\min}$ is as in~\eqref{def:cmin}. Consider the following set, % (\textcolor{green}{Good Set 2: $\cG_2(t)$}),
\begin{align*}
\cG_2(t) := \left\{ \omega: N(t) > (p_{\min} -  \delta_1) t \right\}. 
\end{align*}
We then have that 
\begin{align*}
\bP(\cG^{c}_2(t) ) \le \exp\left( -\delta_1 t  \right). 
\end{align*}
\end{lemma}
\begin{proof}
Consider the following martingale difference sequence $m(i)= \bE\left\{c(i)\big| \cF_{i-1}  \right\}  - c(t) $. Since $\bE\left\{c(i)\big| \cF_{i-1}  \right\}  \ge p_{\min} $, we have that
\begin{align}\label{ineq:1}
\sum_{i=1}^{t} m(i) \ge c_{\min} t - N(t).
\end{align}
Since $|m(i)|\le 1$, we have the following from Azuma-Hoeffding's inequality~\cite{hoeffding1994probability},
\begin{align*}
\bP\left(  \Big|\sum_{i=1}^{t} m(i)\Big|  \ge x  \right) \le \exp\left( -\frac{x^{2}}{t}  \right).
\end{align*}
Letting $x= \delta_1 t$, we get the following,
\begin{align}\label{ineq:2}
\bP\left(  \Big|\sum_{i=1}^{t} m(i)\Big|  \ge \delta_1 t  \right) \le \exp\left( -\delta_1 t  \right).
\end{align}
Substituting~\eqref{ineq:1} into the above inequality, we obtain 
\begin{align*}
\bP\left(  N(t)   \le ( p_{\min} -\delta_1) t   \right) \le \exp\left( -\delta_1 t  \right).
\end{align*}
This completes the proof. 
\end{proof}


\textit{Regret Decomposition}: We now show how we can decompose the regret, and analyze the cumulative regret $R(H)$ of~\eqref{def:regret} by separately analyzing the ``episodic regrets'' $R^{(e)}(k)$:
\begin{align}
\bE\left[R(H)\right] &= \sum_{k=1}^{K} \bE\left[~R^{(e)}(k) \right],\label{reg:dec_1}\\
\mbox{ where } R^{(e)}(k) :&= \bE\left\{\sum_{t\in \cE_k}g(x(t)) - \bar{\Delta}^{\text{w-peak}}(\mathbf{r}^{\star}) \Big|  \cF_{\tau_k} \right\}. \label{reg:dec_2}
\end{align}
Since within $\cE_k$ our learning algorithm employs a stationary controller that depends only upon $\hat{\te}(\tau_k)$, we have that $R^{(e)}(k)$ is a function of $\hat{\theta}(\tau_k)$. We further consider the following two possibilities:\\
Case a) $|\te\ust - \hat{\te}(\tau_k)|< \delta$:  It follows from Lemma~\ref{lemma:convergence} that
\begin{align*}
|R^{(e)}(k)| \le L\left(\tau_{k+1} - \tau_k \right) |\te\ust - \hat{\te}(\tau_k)|,
\end{align*}
Case b) $|\te\ust - \hat{\te}(\tau_k)|> \delta$: It follows from Assumption~\ref{assum:2} that the average performance cannot exceed $K_2$, and hence we can upper-bound $|R^{(e)}(k)|$ by $K_2 \left(\tau_{k+1} - \tau_k \right)$. \par
Upon combining the bounds obtained in Case a) and Case b), we obtain the following result.
\begin{lemma}\label{lemma:regret_decompose}
The cumulative expected regret~\eqref{reg:dec_1} can be upper-bounded as follows,
\begin{align}
&\bE \left[R(H) \right]\le K_2 \sum_{k=1}^{K} \left(\tau_{k+1} - \tau_k  \right) \bP( | \hat{\te}(\tau_k) - \te\ust |>\delta ) \notag\\
&+L \sum_{k=1}^{N} (\tau_{k+1} - \tau_k) \bE \left(  | \hat{\te}(\tau_k) - \te\ust |\id\left\{| \hat{\te}(\tau_k) - \te\ust |\le \delta \right\} \right).\label{def:reg_dec}
\end{align}
\end{lemma}
We now upper-bound each of the two summations separately.
\begin{flushleft}
\emph{First Summation}: 
\end{flushleft}
Choose a sufficiently large $k_0\in \bN$. It follows from Lemma~\ref{lemma:g2} that on a set $\cG_3$ that has a probability greater than $1- \sum_{k>k_0} \exp(-\delta_1 \tau_k)$, the number of samples of $\te\ust$ at the beginning of each episode $k>k_0$ is greater than $\left(p_{\min} -  \delta_1\right)\tau_k$. Thus on $\cG_3$, the radius of $\cC(\tau_k),k>k_0$ is less than $\sqrt{\frac{\log H^{\gamma}}{(p_{\min}- \delta_1)\tau_k }}$. Let $k_1$ be the smallest integer greater than $k_0$ that satisfies
\begin{align}\label{ineq:radius}
\frac{\log H^{\gamma}}{( p_{\min} - \delta_1)\tau_{k_{1} }}\le \delta^{2}.
\end{align} 
Moreover, on the set $\cap_{k}\cG_1(\tau_k)$ the confidence intervals~\eqref{def:ucb_ci} at the beginning of each episode are true. Hence, on the set $\cap_{k}\cG_1(\tau_k) \cap \cG_3$ we have that for $k>k_1$, $| \hat{\te}(\tau_k) - \te\ust |<\delta$. Thus, in case the confidence intervals are true, the summation is bounded by $K_2 \frac{\log H^{\gamma}}{( p_{\min} - \delta_1) \delta^{2}}$. 
From Lemma~\ref{lemma:g1} we have that the probability of failure of confidence interval at $\tau_k$ is less than $\frac{1}{\tau^{\gamma -1}_k}$ and also since $(\tau_{k+1} - \tau_k )\le \tau_k$, we have that the expected regret in the event of a failure is less than $K_2 \frac{1}{\tau^{\gamma - 2}_k}$. Since $\gamma>3$, the summation of this regret over $k$ is finite. In summary, the first summation in~\eqref{def:reg_dec} is upper-bounded by $K_2\frac{\log H^{\gamma}}{( p_{\min} - \delta_1)  \delta^{2}}$.
 
\begin{flushleft}
\emph{Second Summation}: 
\end{flushleft}
We have that for episodes in which $k>k_1$ that the distance $|\te(\tau_k) -\te\ust|$ is upper-bounded by $\delta$. Thus, the summation can be upper-bounded as (after ignoring the constant multiplicative factor of $L$),
\begin{align*}
\sum_{k>k_1} \left(\tau_{k+1}-\tau_k\right) \sqrt{\frac{\log H^{\gamma}}{( p_{\min} - \delta_1)\tau_k }} \le \sqrt{\frac{\log H^{\gamma}}{ ( p_{\min} - \delta_1) }  } \sum_{k>k_1}  \sqrt{\tau_k},
\end{align*}
where the second inequality follows since we have that $\tau_{k+1} - \tau_k \le \tau_k$. By using Cauchy Schwart'z inequality, the quantity $\sum_{k>k_1}  \sqrt{\tau_k}$ can be upper-bounded as $\sqrt{H\log K}$. In summary, the second summation is upper-bounded by 
\begin{align*}
L\sqrt{\frac{\log H^{\gamma}}{ ( p_{\min} - \delta_1) }  } \sqrt{H\log K}.
\end{align*}
Upon combining the bounds on the two summations above, we obtain the following result that bounds the regret of the proposed learning algorithm.
\begin{theorem}
Consider the problem of adaptively choosing the rates $\br(t)$ in order to minimize the cumulative peak age of $M$ sources. Also assume that the statistics of the transmission time $T$ are unknown to the scheduler, and Algorithm~\ref{algo:ucb} is deployed in order to learn the unknown mean transmission time and design $\br(t)$ adaptively. We then have that the cumulative regret can be bounded as follows,
\begin{align*}
\bE\left[R(H)\right] &\le K_2  \frac{\log H^{\gamma}}{( p_{\min} - \delta_1)  \delta^{2}}+ L\sqrt{\frac{\log H^{\gamma}}{ ( p_{\min} - \delta_1) }  } \sqrt{H\log K},
\end{align*} 
where $H$ is the operating time horizon.
\end{theorem}






%\section{Learning}\label{sec:learning}
%The algorithms derived in the previous sections assumed that the users had knowledge of the sensing time $t_s$ and average transmission time $\mathbb{E}[T]$. However, in real-world applications, the transmission and sensing times of users depend upon the surrounding environments, and hence such an assumption is not justified. In this section we assume that $t_s,\mathbb{E}[T]$ are unknown and the goal is to devise an algorithm that ``learns" them in order to use the estimates for solving~\eqref{problem1}. We will only be interested in finite sample guarantees, i.e., what performance guarantees can be provided when the learning algorithm uses only finitely many samples for estimating  $\mathbb{E}[T]$.
%
%Let $\hat{\mathbb{E}}[T]$ denote the estimate of $\mathbb{E}[T]$ from $N$ transmission times samples $\{ T_i \}_{i=1}^{N}$,
%\begin{align}\label{eq:est_T}
%\hat{\mathbb{E}}[T]:= \frac{\sum_{i=1}^{N} T_i}{N(t)}.
%\end{align} 
%It then follows that 
%\begin{align}\label{eq:chernoff}
%\mathbb{P}\left( |\hat{\mathbb{E}}[T] - \mathbb{E}[T] |>\epsilon \right) \leq e^{-N\epsilon^2 }.
%\end{align}
%Let $\hat{r}^{\star}_{l}(t)$ denote an estimate of the optimal rates obtained by plugging in the estimate $\hat{\mathbb{E}}[T]$ in the relation~\eqref{r_f_b_gr_1}.
%\footnote{Note that since the average transmission time is common to all users, the estimate $\hat{\mathbb{E}}[T](t)$ can be calculated by the AP if the users communicate their transmission times to it.}
%\begin{lemma}\label{lemma:learn_1}
%Let $\epsilon,\delta>0$ be user-provided parameters. If the number of samples $N$ used to estimate the transmission time is larger than $N(\epsilon,\delta):= \frac{ \log(1\slash \delta )  }{\epsilon^2}$, then 
%\begin{align}\label{eq:chernoff_1}
%\mathbb{P}\left( |\hat{\mathbb{E}}[T] - \mathbb{E}[T] |>\epsilon \right) \leq \delta .
%\end{align}
%Consequently, for values of $N$ larger than $N(\epsilon,\delta)$, we have
%\begin{align}\label{eq:chernoff_2}
%\mathbb{P}\left( |\hat{r}^{\star}_{l}- \hat{r}^{\star}_{l} |>\kappa \epsilon \right) \leq \delta,
%\end{align}
%where $\kappa = $.
%\end{lemma}
%Since with a high probability the estimate $\mathbf{\hat{r}}^{\star}$ is close to the true optima $\mathbf{r}^{\star}$, we would expect the average age incurred by using $\mathbf{\hat{r}}^{\star}$ should be nearly optimal. This is shown next.
%
%\emph{Performance Analysis of CSMA under $\mathbf{\hat{r}}^{\star}$}\\ 
%In order to analyze the evolution of ages of users in the CSMA system, we will sample the continuous-time process at time instants when either a packet transmission or a packet collision occurs.~This gives us an equivalent \emph{discrete-time} Markov chain in which the state of the system at time $t$, denoted $\mathbf{x}(t)$ is equal to the age values of all the users. We notice that the state-space is equal to $\mathbb{R}^{M}$, and hence is uncountable and non-compact. This is in departure with the existing works in the machine learning community~\cite{DBLP:journals/ftml/BubeckC12} which restrict the study of learning algorithms solely to discrete, finite spaces. 
%
%Denote the transition probability kernel of the Markov chain $\mathbf{x}(t)$ by $P_{\mathbf{r}}( \mathbf{y} | \mathbf{x} )$, where the sub-script denotes its dependence upon the rate vector $\mathbf{r}$. Consider $M$ exponentially distributed random variables.
%
%The transition probabilities are described as
%\begin{align*}
%P_{\mathbf{r}}( \mathbf{y} | \mathbf{x} ) = q \left(\mathbf{x} + \mathbf{1} \mathcal{R}_1 \right) + \sum_{i=1}^{M} p_i \left(   \right)
%\end{align*}
%where $p_1$
%\textbf{Note:Verify from Ahmed}: only two events can occurr:\\
%a) min r + service time, if collision\\
%b) if no collision then min r becomes equal to service time and the remaining increase by min r + service time.
%
%
%Let $V_{t}(\mathbf{x})$ denote the cumulative average age incurred by the system starting in age $\mathbf{x}$ and evolving for time-duration $t$ under the rate vector set equal to $\mathbf{r}$. Similarly $\tilde{V}_{t}(\mathbf{x})$
%
%
%
%\begin{lemma}\label{lemma:learn_2}
%Consider CSMA rate vectors $\mathbf{r},\mathbf{\tilde{r}}$ that satisfy 
%\begin{align}\label{eq:condit_1}
%|P_{\mathbf{r}}( \cdot | \mathbf{x} ) - P_{\mathbf{\tilde{r}}}( \cdot | \mathbf{x} ) | \leq \epsilon P_{\mathbf{r}}( \cdot | \mathbf{x} ), \forall \mathbf{x}.
%\end{align}  
%Then,
%\begin{align*}
%| V_t(\mathbf{x}) - \tilde{V}_t(\mathbf{x})   | \leq \epsilon V_t(\mathbf{x}).
%\end{align*}
%\end{lemma}
%\proofname \\We have
%\begin{align*}
%V_{t+1}(\mathbf{x}) & =  C_{t+1}( \mathbf{x} ) + \int_{\mathbf{y}} V_{t}(\mathbf{x}) P_{\mathbf{r}}( \mathbf{y} | \mathbf{x} ) \mathrm{d} \mathbf{x} \\
%\tilde{V}_{t+1}(\mathbf{x}) & =  C_{t+1}( \mathbf{x} ) + \int_{\mathbf{y}} \tilde{V}_t(\mathbf{x})  P_{\mathbf{\tilde{r}}}( \mathbf{y} | \mathbf{x} ) \mathrm{d} \mathbf{x}.
%\end{align*}
%Subtracting the above equalities for $t=0$ yields
%\begin{align*}
%| V_1(\mathbf{x}) - \tilde{V}_1(\mathbf{x}) |  = \epsilon \bar{V}_{0}(\mathbf{x}). 
%\end{align*}
%Now assume we have $| V_{t}(\mathbf{x}) - \tilde{V}_{t}(\mathbf{x}) |   \leq  \epsilon c_t t$.
%
%For times $t\neq 1$, subtracting the two equations, we obtain
%\begin{align}\label{eq:backward_recursion}
%| V_{t+1}(\mathbf{x}) - \tilde{V}_{t+1}(\mathbf{x}) | & \leq  \epsilon \bar{V}_{t}(\mathbf{x}) + \int |V_t(\mathbf{y}) - \tilde{V}_{t}(\mathbf{y}) |    P_{\mathbf{r}}( \mathbf{y} | \mathbf{x} ) \mathrm{d} \mathbf{x}\notag\\
%&\leq \epsilon M t + c_t \epsilon t \notag\\
%&= (M + c_t) \epsilon t,
%\end{align}
%and hence the coefficients $c_t$ satisfy the recursion
%\begin{align*}
%c_{t+1} = M + c_t,
%\end{align*}
%so that $C_T = M T$, and hence $| V_{T}(\mathbf{x}) - \tilde{V}_{T}(\mathbf{x}) |\leq MT $. Dividing the inequality by time $T$, we obtain the desired result.
%
%\begin{theorem}\label{th:pac_bound}
%The average peak age performance under the CSMA swc using $\mathbf{\hat{r}}^{\star}$ is within $\epsilon M$ of the optimal performance.
%\end{theorem}

